Bridge trisections in rational surfaces

We study smooth isotopy classes of complex curves in complex surfaces from the perspective of the theory of bridge trisections, with a special focus on curves in $\mathbb{CP}^2$ and $\mathbb{CP}^1\times\mathbb{CP}^1$. We are especially interested in bridge trisections and trisections that are as simple as possible, which we call "efficient". We show that any curve in $\mathbb{CP}^2$ or $\mathbb{CP}^1\times\mathbb{CP}^1$ admits an efficient bridge trisection. Because bridge trisections and trisections are nicely related via branched covering operations, we are able to give many examples of complex surfaces that admit efficient trisections. Among these are hypersurfaces in $\mathbb{CP}^3$, the elliptic surfaces $E(n)$, the Horikawa surfaces $H(n)$, and complete intersections of hypersurfaces in $\mathbb{CP}^N$. As a corollary, we observe that, in many cases, manifolds that are homeomorphic but not diffeomorphic have the same trisection genus, which is consistent with the conjecture that trisection genus is additive under connected sum. We give many trisection diagrams to illustrate our examples.

==> Horikawatex.tex <==
There is a related family of complex surfaces obtained by taking the double branched cover over a disconnected surface homologous to $\cC_{6,2n}$.  As in ?, we can view $S^2 \times S^2$ as the Hirzebruch surface $\FF_{2n}$, obtained by projectivizing the bundle $\underline{\CC} \oplus L_{2n}$ over $\CP^1$.  Let $\cS_{2n,0}$ denote the image of the 0-section and let $\cS_{2n,\infty}$ be the infinity section.  The curves $\cS_{2n,0}$ and $\cS_{2n,\infty}$ are disjoint with self-intersection numbers
$$ \cS_{2n,0} \cdot  \cS_{2n,0}= 2n \qquad \text{and} \qquad \cS_{2n,\infty} \cdot \cS_{2n,\infty}= -2n.$$
The surface $5 \cdot \cS_{2n,0}$ can also be represented by a nonsingular complex curve.  Let $\cB_{2n}$ denote the union of $5 \cdot \cS_{2n,0}$ and $\cS_{2n,\infty}$.  

Define $H'(n)$ to be the double branched cover of the pair $(\FF_{2n+2},\cB_{2n+2})$.  

\begin{proposition}
\label{prop:Horikawa-prime-char-numbers}
The surface $H'(n)$ has characteristic numbers
\begin{align*}
c_1^2(H(n)) &= 8n - 8 & c_2(H(n)) &=  40n - 4\\
\sigma(H(n)) &= -24n & \chi_h(H(n)) &= 4n - 1
\end{align*}
The intersection form of $H'(n)$ is odd if and only iff $n \equiv 1$ mod $2$.
\end{proposition}

Combining Freeman's Theorem~\cite{Freedman} with Propositions \ref{prop:Horikawa-char-numbers} and \ref{prop:Horikawa-prime-char-numbers} yields an immediate corollary.

\begin{corollary}
\label{cor:horikawa-homeomorphic}
The manifolds $H'(n)$ and $H(2n)$ are homeomorphic for odd $n \geq 1$.
\end{corollary}

\begin{proposition}
The manifolds $H'(1)$ and $H(2)$ are not diffeomorphic.
\end{proposition}

\begin{proof}
By construction, there is a diffeomorphism
$$ H(2) = \cX_{6,4} \cong \cX_{4,6} \cong E(3),$$
so $H(2)$ is minimal.  However, the preimage of the infinity section $\cS_{2,0}$, which is a sphere of self-intersection $-2$, is a sphere of self-intersection $-1$.  Hence $H'(1)$ is not minimal.
\end{proof}

In general, it is unknown whether $H(2n)$ and $H'(n)$ are an exotic pair for any odd $n \geq 3$.  When $n$ is odd, the surfaces $H(2n)$ and $H'(n)$ are homeomorphic by Freedman's theorem.  However, Horikawa has shown that $H(2n)$ and $H'(n)$ are not deformation equivalent as complex surfaces.  When $n = 1$, we have that $H(2) \cong H'(1) \cong E(3)$.  However, it is unknown in general whether $H(2n)$ and $H'(n)$ are diffeomorphic.  In particular, they are both surfaces of general type, hence the canonical class is the only Seiberg-Witten basic class.

According to ?, the pair $(\FF_{2n+2},\cB_{2n+2})$ admits an efficient generalized bridge trisection.  However, since the curve $\cB_{2n+2}$ is disconnected, the resulting trisection of the double branched cover is inefficient.

\begin{theorem}
The surface $H'(n)$ admits an inefficient $(g,1)$ trisection with $$g = 40n  - 3. $$
\end{theorem} 

When $n = 3$, we see that $\chi(H(6)) = 116$ and $\sigma(H(6)) = -72$.

\begin{theorem}
The surface $H(6)$ admits a $(114,0)$-trisection and the surface $H'(3)$ admits a $(117,1)$-trisection.
\end{theorem}
